Measuring Cosmic Neutrino Masses Independently of Dark Energy

Neutrino oscillations establish that neutrinos are massive, providing the only laboratory detection of physics beyond the Standard Model. Direct kinematic experiments bound the electron-neutrino mass to $m_{\nu_e} < 0.45$ eV (KATRIN, 90% CL), implying $\sum m_\nu \lesssim 1.3$ eV. Conversely, cosmology within $\Lambda$CDM is highly constraining: Planck CMB, CMB lensing, and DESI DR2 BAO yield $\sum m_\nu < 0.056$ eV (95% CL), in 2-3$\sigma$ tension with the inverted-ordering floor (0.10 eV). However, this bound relies on $\Lambda$CDM, while data hint at an evolving dark energy. To determine the model dependence of cosmic neutrino mass bounds, we deconstruct each probe's sensitivity to late-time physics and pursue two robust routes to a $\sum m_\nu$ bound: (i) The existing dark-energy-marginalized route, retaining all data and marginalizing over $(w_0, w_a)$, is shown to also be immune to flexible binned and cubic $w(a)$ histories, yielding $\sum m_\nu < 0.152$ eV, sharpening to $\sigma(\sum m_\nu) \approx 0.043$ eV with Simons Observatory lensing and Spec-S5 BAO. (ii) A new late-Universe-free route combines primary CMB, marginalizing over acoustic-peak smoothing via $A_{\rm lens}$, with the reconstructed lensing spectrum $C_L^{\kappa\kappa}$, removing late-time expansion dependence by construction. This yields $\sum m_\nu < 0.41$ eV today, tightening to 0.31 eV (Simons Observatory) and 0.28 eV (cosmic-variance limit) across all tested dark-energy models. These relaxed bounds trade statistical power for model independence. Interestingly, they land in the sensitivity range targeted by next-generation laboratory experiments like Project 8 ($m_{\nu_e} \sim 0.1$ eV), motivating vital synergies between future cosmological and terrestrial neutrino measurements.

==> acknowledgement.tex <==


Computations were performed on the Niagara supercomputer at the SciNet HPC Consortium. SciNet is funded by Innovation, Science and Economic Development Canada; the Digital Research Alliance of Canada; the Ontario Research Fund: Research Excellence; and the University of Toronto.
